Planetary parameters, XUV environments and mass-loss rates for nearby gaseous planets with X-ray detected host-stars

We leverage Gaia DR2 parallactic distances to deliver new or revised estimates of planetary parameters and X-ray irradiation for a distance-limited ($\lesssim 100$ pc) sample of 27 gaseous planets (from super-Earths to hot Jupiters) with publicly available Chandra and/or XMM observations, for which we carry out a homogeneous data reduction. For 20 planets with X-ray detected host stars we make use of the photoionization hydrodynamics code ATES to derive updated atmospheric mass outflow rates. The newly derived masses/radii are not consistent with the exoplanet.eu values for five systems; HD 149026b and WASP-38, for mass; and Au Mic b, HAT-P-20 and HAT-P-2 for radii. Notably, the lower mass implies a (Saturn-like) density of $0.86\pm 0.09$ g cm$^{-3}$ for HD 149026 b. This independent estimate is consistent with the lowest values reported in the literature. Separately, we report on the X-ray detection of GJ 9827, HD 219134 and LHS 1140 for the first time. The inferred stellar X-ray luminosity of LHS 1140 ($1.34^{+0.19}_{-0.21} \times 10^{26}$ erg sec$^{-1}$) implies that LHS 1140 b is the least irradiated transiting super-Earth known to orbit within the habitable zone of a nearby M-dwarf.

==> table.tex <==

  
  Host Name (1) Host luminosity, solar units (1), upper uncertainty in Lum (1), Lower uncertainty in Lum (1), Host radius, solar units (1), Upper uncertainty in Lum (1), Lower uncertainty in Lum, Teff   Host effective temperature (1)
GJ 436 non c'è
HAT-P-11                   0.273  +0.000  -0.000  0.769 +0.037  -0.048 4757. 
WASP-43                    0.136  +0.001  -0.001  0.663 +0.070  -0.040 4306. 
HD 97658                   0.364  +0.001  -0.001  0.746 +0.016  -0.034 5192. 
55 cnc non c'è
WASP-80                    0.091  +0.000  -0.000  0.606 +0.016  -0.049 4076
GJ1214           non c'è
WASP-69                    0.341  +0.001  -0.001  0.818 +0.025  -0.027 4875.  				GJ9827           non c'è
LHS 1140   solo teff                                                   3872. 
HD 149026                  2.644  +0.010  -0.010  1.468 +0.037  -0.050 6076.
HD 189733                  0.347  +0.000  -0.000  0.780 +0.017  -0.024 5015. 
HD 209458                  1.705  +0.006  -0.006  1.178 +0.010  -0.009 6077.  
HAT-P-20                   0.194  +0.001  -0.001  0.725 +0.041  -0.072 4500.		
WASP-8                     0.876  +0.005  -0.005  0.991 +0.030  -0.006 5610.  			
GJ 3470                                                                3776. 
WASP-38                    2.838  +0.024  -0.024  1.474 +0.060  -0.066 6170.            
WASP-77 A                  0.770  +0.010  -0.010  0.947 +0.030  -0.042 5556. 
WASP-10                    0.229  +0.002  -0.002  0.670 +0.042  -0.045 4878.
WASP-18                    2.414  +0.013  -0.013  1.240 +0.077  -0.120 6462. 


Planet  Planet Name, Planet Radius, Upper uncertainty in Rad, Lower uncertainty in Rad, Planet Mass (1), Upper uncertainty in Mass, Lower uncertainty in Mass, Planet Density, Upper uncertainty in rho, Lower uncertainty in rho, Semi-major axis (1), Upper uncertainty in a, Lower uncertainty in a, Planet Incident Flux, Upper uncertainty in Sinc, Lower uncertainty in Sinc
                          Planet radius           
Gj 436
HAT-P-11 b                0.428 +0.038 -0.041  0.090  +0.010  -0.010  1.423  +0.411  -0.443
WASP-43 b                 1.033 +0.183 -0.198  1.780  +0.100  -0.100  2.005  +1.071  -1.161   0.014  +0.000  -0.000   674.951   +19.388   
HD 97658 b                0.216 +0.017 -0.019  0.030  +0.000  -0.000  3.697  +0.881  -0.985 55 cnc
WASP-80 b                 1.029 +0.065 -0.101  0.538  +0.035  -0.036  0.612  +0.123  -0.185   0.034  +0.001  -0.001    77.074    +2.255 
Gj 1214
WASP-69 b                 1.056 +0.065 -0.066  0.290  +0.030  -0.030  0.306  +0.065  -0.066      
GJ9827           non c'è
LHS 1140 non c'è
HD 149026 b               0.770 +0.031 -0.036  0.380  +0.060  -0.060  1.032  +0.206  -0.219                                    
HD 189733 b               1.175 +0.030 -0.039  1.130  +0.080  -0.080  0.865  +0.090  -0.106                        
HD 209458 b               1.378 +0.028 -0.027  0.730  +0.040  -0.040  0.346  +0.028  -0.028                                     
HAT-P-20 b                0.911 +0.075 -0.105  7.246  +0.187  -0.187 11.890  +2.939  -4.125   0.036  +0.001  -0.001   149.237    +2.162      
WASP-8 b                  1.086 +0.073 -0.066  2.540  +0.330  -0.330  2.458  +0.590  -0.548                                                        
WASP-8 c                                                                                      5.280  +0.630  -0.340     0.031    +0.004         
gj 3470 non c'è
WASP-38 b                 1.190 +0.083 -0.086  3.440  +0.360  -0.360  2.534  +0.595  -0.610                 
WASP-77 A b               1.201 +0.110 -0.116  2.290  +0.330  -0.330  1.637  +0.508  -0.531                                       
WASP-10 b                 1.034 +0.073 -0.077  3.150  +0.130  -0.110  3.531  +0.759  -0.800   0.038  +0.001  -0.000   160.139    +3.106 
WASP-18 b                 1.151 +0.093 -0.126 11.440  +1.510  -1.510  9.309  +2.567  -3.303                                     


Da d*, misurando una magnitudine relativa, si trova una magnitudine assoluta (dal quale si può stimare una luminosità bolometrica totale, Gaia lo fa). Se si hanno diverse stime di magnitudine relativa si stima Teff (Gaia ha un sotware sviluppato da Andrae et al. (2018) che lo fa direttamente). 

- Da queste stime di L e Rstar si può stimare R star con stephan boltzman. 
- In alcuni casi invece di percorrere questa strada da Lstar si usano delle mass luminosity relation specifiche per ogni classe spettrale per ricavare Mstar.
                    - successiamente o si usa una Mass-radius relation per stimare Mstar
                    - oppure da Mstar e da P (transito o radial velocity) si stima con Keplero a 
                      una volta stimato a, dalla durata del transito si stima direttamente a/Rstar. Quindi si ricava Rstar così. 
                      
Per Mp invece c'è la formulona. 

